Quadratic Functional Encryption for Secure Training in Vertical Federated Learning

Vertical federated learning (VFL) enables the collaborative training of machine learning (ML) models in settings where the data is distributed amongst multiple parties who wish to protect the privacy of their individual data. Notably, in VFL, the labels are available to a single party and the complete feature set is formed only when data from all parties is combined. Recently, Xu et al. proposed a new framework called FedV for secure gradient computation for VFL using multi-input functional encryption. In this work, we explain how some of the information leakage in Xu et al. can be avoided by using Quadratic functional encryption when training generalized linear models for vertical federated learning.

==> ModifiedAlgoForTraining.tex <==
 \begin{algorithm}
\caption{Training Procedure} 
\label{alg:training}
\begin{algorithmic}[1]
\Procedure{Training-Aggregator}{$\mathbold{w}^t,s,\{F_i\}_{i=0}^{N-1},N$}
    % \State Divide $\mathbold{w}^t$ into $\{\mathbold{w}_{i}^t\}_{i=0}^{N-1}$ 
    \State $\mathbold{res} = \textbf{0}^{F}$
    \State $\mathcal{C}^t:=\{\mathbold{C}^t_{i,p}, i\in [N],p \in [F_{i}]\}$
    \ForEach{$n \in {0,...,N-1}$}
    \ForEach{$p \in {0,...,F_{n}-1}$}
    \State $\mathbold{C}_{i,p}^t :=$ CGEN($\mathbold{w}^t,s,{F},N,i,p$)
    \EndFor
    \EndFor
    \State $\{\{\qmife.\sk_{\textbf{C}_i^t}\}_{p=0}^{F_i}\}_{i=0}^{N-1}= \textsf{obtain-dk-from-TTP}(\mathcal{C}^t)$
    \ForEach{$i \in {0,...,N-1}$}
    \If{party $i$ has label $\mathbold{y}^t$} 
    \State ($ct_i^t,ct_y^t$)= \textsf{obtain-ct-from-client()}
    \Else
    \State $ct_i^t$ = \textsf{obtain-ct-from-client()}
    \EndIf
    \EndFor
    \State ${ct}^t =\{\{{ct}^t_{i}\}_{i=0}^{N-1}, {ct}^t_{y}\}$ 
    \ForEach{$n \in {0,...,N-1}$}
    \ForEach{$p \in {0,...,F_{n}-1}$}
        \State \textsf{idx} =  $\sum_{i=0}^{n-1}F_{i}+p$
        % \State ${ct} =\{\{{ct}_{i}\}_{i=0}^{N-1}, {ct}_{y}\}$ 
        \State $\mathbold{res}[\textsf{idx}] =  \qmife.\dec( {ct}^t, \qmife.\sk^t_{\mathcal{C}_{i,p}})$
    \EndFor
    \EndFor
    \State $\nabla L(\mathbold{w}^t) = -\frac{2}{s}\mathbold{res} + \lambda \nabla R(\mathbold{w}^t)$
    \State $\mathbold{w}^{t+1} = \mathbold{w}^t - \alpha \nabla L(\mathbold{w}^t)$
    \EndProcedure
\Procedure{Training-Party}{$\qmife.\ek^t_{i}, \mathbold{X}_{i}^t$}
\Function{obtain-ct-from-client()}{}
    \State $\textbf{x}_{i}^t:= \textsf{vec}({\mathbold{X}_{i}^t}^\top)$ 
    \If{party $i$ has label $\mathbold{y}^t$} 
    \State $\mathbold{ct}_{i}^t:= \qmife.\enc(\qmife.\ek^t_{i}, \textbf{x}_{i}^t)$
    \State  $\mathbold{ct}_{y}^t:= \qmife.\enc(\qmife.\ek_{i}^t, \mathbold{y}^t)$
    \State Return $(\mathbold{ct}^t_{i},\mathbold{ct}_{y}^t)$ to Aggregator 
    \Else 
    \State $\mathbold{ct}_{i}^t:= \qmife.\enc(\qmife.\ek_{i}^t, \textbf{x}_{i}^t)$
    \State Return $\mathbold{ct}^t_{i}$ to Aggregator
    \EndIf
    \EndFunction
    \EndProcedure
\Procedure{Training-TTP}{$\textsf{qMIFE.MSK}$}
    \Function{obtain-dk-from-TTP}{$\mathcal{C}^t$}
    
    $(\pp^t, \{\ek_i\}^t_i, \msk^t) \gets \qmife.\setup(1^\secp, 1^n)$
    \ForEach{$i \in {0,...,N-1}$}
    \ForEach{$p \in {0,...,F_i}$}
    \State $\qmife.\KeyGen(\qmife.\msk^t, \mathbold{C}_{i,p}^t)\rightarrow \qmife.\sk^t_{\mathbold{C}_{i,p}}$
    \EndFor
    \EndFor
    \State Return $\{\{\qmife.\sk^t_{\mathbold{C}_{i,p}}\}_{p=0}^{F_i}\}_{i=0}^{N-1}$
    \EndFunction
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> OldAlgo1.tex <==
\begin{tiny}     
 \begin{algorithm}
\caption{Training Procedure} 
\label{alg:training}
\begin{algorithmic}[1]
\Procedure{Training-Aggregator}{$\mathbold{w}^t,s,\{F_i\}_{i=0}^{N-1},N$}
    % \State Divide $\mathbold{w}^t$ into $\{\mathbold{w}_{i}^t\}_{i=0}^{N-1}$ 
    \State $\mathbold{res} = \textbf{0}^{F}$
    \State $\mathcal{C}^t:=\{\mathbold{C}^t_{i,p}, i\in [N],p \in [F_{i}]\}$
    \ForEach{$n \in {0,...,N-1}$}
    \ForEach{$p \in {0,...,F_{n}-1}$}
    \State $\mathbold{C}_{i,p}^t :=$ CGEN($\mathbold{w}^t,s,{F},N,i,p$)
    \EndFor
    \EndFor
    \State $\{\{\textsf{DK}_{\textbf{C}_i^t}\}_{p=0}^{F_i}\}_{i=0}^{N-1}= \textsf{obtain-dk-from-TTP}(\mathcal{C}^t)$
    \ForEach{$i \in {0,...,N-1}$}
    \If{party $i$ has label $\mathbold{y}^t$} 
    \State ($\textsf{CT}_i^t,\textsf{CT}_y^t$)= \textsf{obtain-ct-from-client()}
    \Else
    \State $\textsf{CT}_i^t$ = \textsf{obtain-ct-from-client()}
    \EndIf
    \EndFor
    \State ${\textsf{CT}}^t =\{\{{\textsf{CT}}^t_{i}\}_{i=0}^{N-1}, {\textsf{CT}}^t_{y}\}$ 
    \ForEach{$n \in {0,...,N-1}$}
    \ForEach{$p \in {0,...,F_{n}-1}$}
        \State \textsf{idx} =  $\sum_{i=0}^{n-1}F_{i}+p$
        % \State ${ct} =\{\{{ct}_{i}\}_{i=0}^{N-1}, {ct}_{y}\}$ 
        \State $\mathbold{res}[\textsf{idx}] =  \textsf{Dec}(\textsf{DK}^t_{\mathcal{C}_{i,p}}, {\textsf{CT}}^t)$
    \EndFor
    \EndFor
    \State $\nabla L(\mathbold{w}^t) = -\frac{2}{s}\mathbold{res} + \lambda \nabla R(\mathbold{w}^t)$
    \State $\mathbold{w}^{t+1} = \mathbold{w}^t - \alpha \nabla L(\mathbold{w}^t)$
    \EndProcedure
\Procedure{Training-Party}{$\textsf{EK}_{i}, \mathbold{X}_{i}^t$}
\Function{obtain-ct-from-client()}{}
    \State $\textbf{x}_{i}^t:= \textsf{vec}({\mathbold{X}_{i}^t}^\top)$ 
    \If{party $i$ has label $\mathbold{y}^t$} 
    \State ${\textsf{CT}}_{i}^t:= \textsf{Enc}(\textbf{x}_{i}^t,\textsf{EK}_{i})$
    \State  ${\textsf{CT}}_{y}^t:= \textsf{Enc}(\mathbold{y}^t,\textsf{EK}_{i})$
    \State Return $({\textsf{CT}}^t_{i},{\textsf{CT}}_{y}^t)$ to Aggregator 
    \Else 
    \State ${\textsf{CT}}_{i}^t:= \textsf{Enc}(\textbf{x}_{i}^t,\textsf{EK}_{i})$
    \State Return ${\textsf{CT}}^t_{i}$ to Aggregator
    \EndIf
    \EndFunction
    \EndProcedure
\Procedure{Training-TTP}{$\textsf{MSK}$}
    \Function{obtain-dk-from-TTP}{$\mathcal{C}^t$}
    \ForEach{$i \in {0,...,N-1}$}
    \ForEach{$p \in {0,...,F_i}$}
    \State \textsf{KeyGen}$(\mathbold{C}_{i,p}^t,\textsf{MSK})\rightarrow \textsf{DK}_{\mathbold{C}_{i,p}}^t$
    \EndFor
    \EndFor
    \State Return $\{\{\textsf{DK}^t_{\mathbold{C}_{i,p}}\}_{p=0}^{F_i}\}_{i=0}^{N-1}$
    \EndFunction
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
 \end{tiny}

 

==> Tagged-MIFE.tex <==
\section{Secret-Key Multi-Input Tagged Functional Encryption}
\label{app:tfe}

The notion of Tagged Functional Encryption (TFE) was introduced by Garg et. al. \cite{GGLW22}. This notion is the same as Functional Encryption with the only difference being that the decryption is successful when the \textit{tags} associated with ciphertext and the secret keys match. \cite{GGLW22} defined the TFE for the single input setting. We generalize the definition for the secret-key setting and define TFE for the multi-input setting.
%\amnote{GGLW22 defines the tagged FE for public key setting. I am writing in the definition for the secret key setting because we need a secret key tagged FE for our case. Please let me know if it is okay.}

\begin{definition}[Secret-key Multi-Input Tagged Functional Encryption ($\tfe$) \amnote{Garg et. al. defined it for single input. I am not including the GGLW22 citation as we are generalizing it to a multi-input setting in this definition. Please let me know if it is important.}]
\label{defi-TFE}
\label{def:TFE}

%Let $\{ \mathcal{F}_N\}_{N \in \mathbb{N}}$ be a family of functional classes, $\{ \mathcal{M}_N\}_{N \in \mathbb{N}}$ be the message spaces and $\{ \mathcal{I}_z\}_{z \in \mathbb{N}}$ be the tag spaces. 

\textbf{Syntax.} Let $N$ be the number of encryption slots, and $\mcF = \{\mcF_N\}_{N \in \mathbb{N}}$ be a function family such that, for all $f \in \mcF_N$, $f: \mcX_{1} \times \cdots \times \mcX_{N} \to \mcY$. Here $\mcX_i$ and $\mcY$ be the input and output spaces (respectively). Let $\{ \mathcal{I}_z\}_{z \in \mathbb{N}}$ be the tag spaces. The tagged FE scheme $\tfe$ consists of four polynomial time algorithms $(\setup, \enc, \KeyGen, \dec)$.

\begin{description}
\item [$\ms{Setup}(1^{\secp}, 1^N, 1^z) \rightarrow (\pp, \{\ek_i\}_{i}, \msk)$.] It takes a security parameter $1^{\secp}$, number of slots $1^N$, a tag space index $z$, which fixes a tag space $\mathcal{I}_z$, and outputs a public parameter $\pp$, $N$ encryption keys $\{\ek_i\}_{i \in [N]}$ and a master secret key $\msk$. (The remaining algorithms
implicitly take $\pp$ as input.) 

%\amnote{I have not included the collusion bound $1^q$ as an input to the Setup algorithm to simplify the notation. Please let me know if it is important.} No, we are anyway not in the bounded collusion setting.

\item [$\enc(\ek_i, \tfetag \in \mathcal{I}_z,  \vecx_i) \rightarrow \ct_i$.] It takes the $i^\text{th}$ encryption key $\ek_i$, a tag $\tfetag \in \mathcal{I}_z$ and an input $\vecx \in \mcX_{i}$, and outputs a ciphertext $\ct_{i}$.

\item [$\KeyGen( \msk, \tfetag \in \mathcal{I}_z, f ) \rightarrow \sk$.] It takes the master secret key $\msk$, a tag $\tfetag \in \mathcal{I}_z$ and function $f \in \mcF$ as inputs, and outputs a secret key $\sk$.

\item [$\dec( \ct_{1} \dada \ct_{N}, \sk) \rightarrow y$.] It takes $n$ ciphertexts $ \ct_{1} \dada \ct_{N}$ and secret key $\sk$, and outputs a decryption value $y \in \mcY$ or a special abort symbol $\bot$.
\end{description}

\noindent{\textbf{Correctness.}}
A $\tfe$ scheme is correct if for all $\secp, N, z \in \mathbb{N}$, every function $f \in \mcF_N$, $(\vecx_{1} \dada \vecx_{N}) \in \mcX_{1} \times \cdots \times \mcX_{N}$, tag $\tfetag \in \mathcal{I}_z$ and $(\pp, \{\ek_i\}_{i}, \msk) \leftarrow \ms{Setup}(1^{\secp}, 1^N, 1^z)$ we have

%$$\Pr[\dec(\enc(\ek_1, \tfetag \in \mathcal{I}_z,  \vecx_1), \ldots, \enc(\ek_N, \tfetag \in \mathcal{I}_z,  \vecx_N), \KeyGen(\msk, \tfetag \in \mathcal{I}_z, f)) = f(m)] = 1$$

{
\footnotesize{
\begin{align*}
\Pr\left[y =f(x_{1} \dada x_{N}) : 
\begin{array}{l}
(\pp, \{\ek_i\}_{i}, \msk) \gets \setup(1^{\secp}, 1^N, 1^z)\\
\Set{\ct_{i} \gets \enc(\ek_i, \tfetag,  \vecx_i)}_{i \in [N]} \\
\sk \gets \KeyGen(\msk, \tfetag, f)\\
y = \dec( \ct_{1}\dada \ct_{N}, \sk)
\end{array}
\right]
= 1.
\end{align*}}}
where the probability is taken over the coins of setup, key generation and encryption algorithms.

%\noindent{\textbf{Security.}} 
\end{definition}

\subsection{Security Definition for TFE}
Intuitively, security says that no information about the messages can be learned by the adversary except what is revealed by virtue of functionality -- in more detail, an adversary possessing some ciphertexts associated with $\tfetag_1$ and secret keys associated with $\tfetag_2$ can perform decryption only when $\tfetag_1 = \tfetag_2$ and learn the output of the functionality, which itself leaks something about the underlying plaintext. But besides this necessary leakage, the adversary does not learn anything.
%\snote{we do not need function hiding.}
\begin{definition}[TFE Security \cite{GGLW22}] \label{def:tfe}
For any choice of parameters $\secp, N, z \in \mathbb{N}$, consider the following list of stateful oracles $\oracle_0, \oracle_1, \oracle_2$ where these oracles simulate the FE setup, key generation, and encryption algorithms respectively, and all three algorithms share and update the same global state of the simulator. Here the attacker interacts with the execution environment $\env$, and the environment makes queries to the simulator oracles. Formally, the simulator oracles and the environment are defined below:

\begin{description}
    \item $\oracle_0(1^\secp, 1^N, 1^z)$ generates the simulated master public key $\mpk$ of the system, and initializes the global state $\st$ of the simulator which is used by the next two oracles.

    \item $\oracle_1(\cdot, \cdot, \cdot)$ upon a call to generate secret key on a function-tag-value tuple $(f_i , \tfetag_i, \mu_i)$, where the function value is either $\mu_i = \bot$ (signalling that the adversary has not yet made any encryption query on tag $\tfetag_i$), or $(x^{\tfetag_i}, \tfetag_i)$ has already been queried for encryption (for some message $x^{\tfetag_i}$), and $\mu_i = f_i(x^{\tfetag_i})$, the oracle outputs a simulated key $\sk_{f_i, \tfetag_i }$.
\end{description}

\amnote{I have a doubt. Should I write what all oracles does formally?}

A tagged functional encryption scheme $\tfe = (\setup, \enc,\KeyGen, \dec)$ is said to be tagged-simulation-secure if there exists a stateful PPT simulator $\simulator = (\oracle_0, \oracle_1, \oracle_2)$ such that for every stateful admissible PPT adversary $\adv$, the following distributions are computationally indistinguishable:

{
\footnotesize{
$$\left \{ \adv^{\KeyGen(\msk, \cdot, \cdot), \enc(\ek_i, \cdot, \cdot)}(\pp):  
\begin{array}{l}
(1^N, 1^z)\leftarrow \adv(1^\secp)\\
(\pp, \{\ek_i\}_{i}, \msk) \gets \setup(1^{\secp}, 1^N, 1^z)
\end{array}
\right \}_{\secp \in \mathbb{N}}
$$
$$
\approx_c
$$
$$
\left \{ \adv^{\env^{\oracle_1, \oracle_2}(\cdot, \cdot)}(\pp):  
\begin{array}{l}
(1^N, 1^z)\leftarrow \adv(1^\secp)\\
\pp \gets \oracle_0(1^{\secp}, 1^N, 1^z)
\end{array}
\right \}_{\secp \in \mathbb{N}}
$$}}

where the adversary $\adv$ is said to be admissible if and only if
\begin{itemize}
    \item $\adv$ makes at most one encryption query per unique tag (that is, if the adversary made an encryption query on some tag $\tfetag_i$ previously, then making another encryption query for the same tag is disallowed)

    \item $\adv$ makes at most $q$ queries combined to the key generation oracles in the above experiments for all tags $\tfetag_i$ such that it also submitted an encryption query for tag $\tfetag_i$.
\end{itemize}
\end{definition}



==> relatedworks.tex <==
\section{Related Work}
Vertical federated learning (VFL) refers to scenarios where parties have the same set of samples but differ in feature space. It promotes collaborative training of ML models among parties with vertically partitioned data. One of the main concerns is data privacy and security. Existing works \cite{Gascn2016SecureLR, Yang2019AQM, Hardy2017PrivateFL, GuDang, Zhang, Wang, Chen} about privacy-preserving protocols make use of privacy enhancement techniques including  homomorphic encryption (HE) and differential privacy (DP), etc. 

Differential Privacy is an approach relying on adding noise to the original data to preserve the privacy. Wang et al. \cite{Wang} proposed a DP-based protocol to ensure data confidentiality. However, DP noise will degrade the prediction accuracy of the model. 
